Decentralized LTL Enforcement

We consider the runtime enforcement of Linear-time Temporal Logic formulas on decentralized systems with no central observation point nor authority. A so-called enforcer is attached to each system component and observes its local trace. Should the global trace violate the specification, the enforcers coordinate to correct their local traces. We formalize the decentralized runtime enforcement problem and define the expected properties of enforcers, namely soundness, transparency and optimality. We present two enforcement algorithms. In the first one, the enforcers explore all possible local modifications to find the best global correction. Although this guarantees an optimal correction, it forces the system to synchronize and is more costly, computation and communication wise. In the second one, each enforcer makes a local correction before communicating. The reduced cost of this version comes at the price of the optimality of the enforcer corrections.

==> eptcsdata.tex <==
\providecommand{\firstpage}{135}
\providecommand{\publicationstatus}{D. Bresolin and P. Ganty (Eds.): 12th International Symposium \\
on Games, Automata, Logics, and Formal Verification (GandALF 2021)\\
EPTCS 346, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.346.9}{10.4204/EPTCS.346.9}}
\pdfoutput=1

